A Class of Trees Having Near-Best Balance

Full binary trees naturally represent commutative non-associative products. There are many important examples of these products: finite-precision floating-point addition and NAND gates, among others. Balance in such a tree is highly desirable for efficiency in calculation. The best balance is attained with a divide-and-conquer approach. However, this may not be the optimal solution, since the success of many calculations is dependent on the grouping and ordering of the calculation, for reasons ranging from the avoidance of rounding error, to calculating with varying precision, to the placement of calculation within a heterogeneous system. We introduce a new class of computational trees having near-best balance in terms of the Colless index from mathematical phylogenetics. These trees are easily constructed from the binary decomposition of the number of terms in the problem. They also permit much more flexibility than the optimally balanced divide-and-conquer trees. This gives needed freedom in the grouping and ordering of calculation, and allows intelligent efficiency trade-offs.

==> figs_old/fig_colless_graphs.tex <==
\begin{figure}[H]
    \centering
    \begin{subfigure}{0.48\textwidth} 
        \includegraphics[scale=0.6]{figs/img_minD_log.png}
        \caption{Colless indices on ascending and  descending MinD trees normalized against the minimum and maximum possible Colless indices. The logarithmic scale shows the decrease in terms of $\log_2(n)$. All except a few small $n$  are well below 10\% of the normalized max.}
        \label{fig:colless_minmax_values-a}
    \end{subfigure}
    \hspace{1em}
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[scale=0.6]{figs/img_minD_256_512.png}
        \caption{Here, $\log_2(n)$  is $8$, and already, most of the minD trees have normalized Colless index at less than 2.5\% of the normalized max. \newline\newline\newline}
        \label{fig:colless_minmax_values-b}
    \end{subfigure}
    \mycaption{
    Normalized Colless  indices for MinD trees having minimum and maximum Colless indices} {We normalize these values by the minimum possible Colless index, which is that of the divide-and-conquer tree on $n$ nodes, and the maximum, which is that of the ladder tree. The minimum Colless index for a MinD tree is on the descending ladder base tree, and the maximum is on the ascending ladder base tree. Both of these are quite close to the minimum possible Colless  index, and are decreasing with $\log_2(n)$.}
    \label{fig:colless_minmax_values}
\end{figure}



==> oeis_seqs.tex <==
\noindent (Concerned with sequences
\seqnum{A000992},
\seqnum{A001147},
\seqnum{A001710},
\seqnum{A002620},
\seqnum{A011371},
\seqnum{A048881},\\
\seqnum{A060818},
\seqnum{A049606},
\seqnum{A096351},
\seqnum{A119387},
\seqnum{A268289},
\seqnum{A296062}  and
\seqnum{A335833}.)

